CitySpec: An Intelligent Assistant System for Requirement Specification in Smart Cities

An increasing number of monitoring systems have been developed in smart cities to ensure that real-time operations of a city satisfy safety and performance requirements. However, many existing city requirements are written in English with missing, inaccurate, or ambiguous information. There is a high demand for assisting city policy makers in converting human-specified requirements to machine-understandable formal specifications for monitoring systems. To tackle this limitation, we build CitySpec, the first intelligent assistant system for requirement specification in smart cities. To create CitySpec, we first collect over 1,500 real-world city requirements across different domains from over 100 cities and extract city-specific knowledge to generate a dataset of city vocabulary with 3,061 words. We also build a translation model and enhance it through requirement synthesis and develop a novel online learning framework with validation under uncertainty. The evaluation results on real-world city requirements show that CitySpec increases the sentence-level accuracy of requirement specification from 59.02% to 86.64%, and has strong adaptability to a new city and a new domain (e.g., F1 score for requirements in Seattle increases from 77.6% to 93.75% with online learning).

==> comments.tex <==

Solution: 

[fixed] 1. The first example about something like  “no more than 7 taxis” does not sound like a reasonable example (who would make such a requirement; doesn’t sound real) also the time says something like  7 to 8   --  but no AM or PM
 
2. Why are there 3 language models being tested?  Perhaps add “why” to why we did things etc in various places (there are some instances of this but not in other places)
 
[fixed] 3. What is sent-level
 
4. I don’t have more time today but it seems to be missing something … maybe in places it has a high level of description of the solution only and it never maps back to the effect on city planners which is the main motivation.
 
 


Evaluation: 

[fixed] 5. It seems that the challenges listed in the beginning of the paper and what we are evaluating are not always matching.  For example, can we better “match” sentence accuracy to these challenges?
 
-- yes, let me address this one. Our system got much higher accuracy (sentence accuracy and token accuracy) than using the traditional language models directly.
 
6. Another example, we complain about missing info, ambiguous statements, etc but don’t really highlight those in the evaluation.  We do some of that in terms of ambiguity in relation to “names” but I assume there is a lot more ambiguity than that.
 
--I agree. For now, detecting missing and ambiguous information is through conversation, we only describe it in the solution part. I did not find a good metric to show this dynamic process in the evaluation. Maybe a case study or some examples would work? We also have some results on xx\% of missing/ambiguous location, time, … detected out of all the requirements. we mention it in the solution, maybe we should present it in the evaluation. Let me check.
 
[fixed] 7. Should we explicitly say in the conclusions that we show the “technical” accuracy/value of the tool based on datasets. Future work it to have the solution used by real city managers, but this is outside the scope of this paper?
 
--Yes. I will do that.

8. But even if its use with real city personnel is later we can claim that we are emulating that process by taking the requirements and assuming that they are input by city managers –….maybe it is clear that is how we are using the requirements in the evaluation (do you think it is)?
but of course that does not evaluate a back-and-forth interaction with the cognitive assistant
 

==> dataaugmentation.tex <==
\section{Data Augmentation}
\label{sec:augmentation}
During development, we are faced with a significantly insufficient data source. Although there are over 1,000 sentences in the initial unlabeled dataset, after manual labeling, the number of valid data entries sharply dropped to 316. This small amont of available data makes it more difficult to train a data-hungry model like Bi-LSTM + CRF or even BERT. To mitigate the data scarcity problem, we invent a novel data augmentation solution. 

During our data augmentation process, we need to loop over the whole dataset and main two key structures: one is a list of all \textbf{Pattern}, another one is a dictionary of all named entities and their corresponding \textbf{Vocabulary}.

\subsection{Pattern v.s. Vocabulary}

The term \textbf{Vocabulary} in the proposed Data Augmentation is defined as all the possible options for each predefined named entity. On the other hand, the term \textbf{Pattern} is defined to be similar to initial sentences but all those labeled keywords are replaced by their corresponding labels.

For example, we have the following two sentences, which can be found as the 2nd and the 47th sentence in the original dataset without any augmentation:

Sentence 1: In all \textit{buildings}/\textbf{LocKey}, the average \textit{concentration}/\textbf{Key1} of \textit{TVOC}/\textbf{Key2} should be no more than \textit{0.6 mg/m3}/\textbf{Number} for \textit{every day}/\textbf{Time}.

Sentence 2: The \textit{toluene}/\textbf{Key1} should be less than \textit{0.2 mg per m3}/\textbf{Number} within an hour nearby all \textit{park}/\textbf{LocKey}

By our design, the \textbf{Vocabulary} of current two sentences will be:

\begin{table}[h]
    \centering
        \caption{Domain explanation}
 \begin{tabular}{||c c||} 
 \hline
 Named Entity & Possible Options\\ [0.5ex] 
 \hline\hline
 Key1 & \{`concentration', `toluene'\} \\ 
 \hline
 Key2 & \{`TVOC'\} \\
 \hline
 LocKey & \{`buildings', `park'\} \\
 \hline
 Time & \{`every day'\} \\
 \hline
 Number & \{`0.6 mg/m3', `0.2 mg per m3'\} \\
 \hline
\end{tabular}
    \label{tab:Distance}
\end{table}

And the Pattern in those two sentences will be stored and further maintained as following (`\#' is designed to be a dummy symbol for future detection and location):

Pattern 1: In all \textbf{\#LocKey}, the average \textbf{\#Key1} of \textbf{\#Key2} should be no more than \textbf{\#Number} for \textbf{\#Time}.

Pattern 2: The \textbf{\#Key1} should be less than \textbf{\#Number} within an hour nearby all \textbf{\#LocKey}

\textcolor{blue}{This following paragraph can be moved to later section}

After defining Pattern and Vocabulary, we have 240 possible options in Key1, 173 options in Key2, 117 options in LocKey, 48 samples in Time, 214 options in Number. This relatively small amount of vocabulary is from 316 sentences that are manually validated. To enrich the vocabulary, we go through those excluded requirements to mine all possible options for each domain, although some of them are not validated. After first step of exploitation, we have 295 options in Key1, 306 options in Key2, 273 options in LocKey, 82 options in Time, and 411 options in Number. We also grab 500 more requirements from the code of ordinances from the city government of Nashville, Knoxville and Memphis. After fully exploiting those 500 new requirements, the vocabulary was incremented to have 530 options in Key1, 567 options in Key2, 501 in LocKey, 186 in Time, and 595 in Number. The Time and Number domain often have relatively smaller amount of references compared with other domains. We generate a considerable amount of new samples based on the pattern found in Time and Number domain: (1) all month-related keywords are replaced with other 11 alternative ones, for example `January' to `February' or `Feb'; (2) all city administration-related units are collected and combined with randomly generated float numbers to serve as new options in Number. The change of dataset size is shown in Fig \ref{fig:domain}.

\begin{figure}
    \centering
    \includegraphics[scale=0.35]{Figure/domain_dist.png}
    \caption{Domain distribution}
    \label{fig:domain}
\end{figure}

\subsection{Controllable Augmentation}

Our designed data augmentation approache is called Complete Data Augmentation, see Alg.1. The augmentation index is introduced to control the times of how much bigger the newly augmented dataset will be compared with the dataset volume.


\begin{algorithm}
 \caption{Complete Data Augmentation}
 \begin{algorithmic}[1]
 \renewcommand{\algorithmicrequire}{\textbf{Require:}}
 \REQUIRE $X \notin \varnothing$: initial dataset
 \REQUIRE $V, P = \varnothing$: \textbf{Vocabulary},\textbf{Pattern}
 \REQUIRE $\gamma \in N$: Augmentation Index
 \REQUIRE $L \in N$: Dataset Volume
 \FOR{\texttt{$i \gets 0$; $i \leq L$; $i \gets i + 1$}}
    \STATE $\textbf{Generate} \ V$
    \STATE $\textbf{Generate} \ P$
 \ENDFOR
 \STATE $L = \max(\max(V), \max(P))$
 \STATE Augmented Dataset $\chi = \varnothing$
 \WHILE{$\gamma \neq 0$}
    \FOR{\texttt{<each entry $\eta$ in $V$>}}
        \STATE Randomly shuffle $\eta$
        \STATE Concatenate shuffled $\eta$ together
    \ENDFOR
    \STATE $\gamma \gets \gamma - 1 $
 \ENDWHILE
 \STATE Let $V'$ denotes $V$ after concatenation above
 \STATE \textbf{assert} : The volume of $V' = \gamma * \lambda$ 
 \WHILE{The length of $\chi < \gamma * \lambda$}
    \FOR{\texttt{<each entry $\rho$ in $P$>}}
        \STATE Assign a \texttt{Pointer} to each $\eta'$ in $V'$
         \STATE Iterate within all $\eta'$s to fulfill $\rho$ with options $o$
        \STATE Generate new sentence $x$ based on $\rho$ and option $o$
        \IF{the option $o$ is generated by $\eta''$}
            \IF{The \texttt{Pointer} of $\eta''$ reaches the boundary}
                \STATE Move the \texttt{Pointer} back to the beginning
            \ELSE \STATE Move the \texttt{Pointer} one step forward
            \ENDIF
        \ENDIF
    \STATE Append $x$ to the Augmented Dataset $\chi$
    \ENDFOR
 \ENDWHILE

 \end{algorithmic} 
 \end{algorithm}

In the Complete Data Augmentation algorithm, the augmented dataset will have a size of $\gamma * \lambda$, where the $\gamma$ refers to the augmentation index and the $\lambda$ represents the Dataset Volume. The size of \textbf{Vocabulary} is defined as the maximum length all all its values under each keys. The size of \textbf{Pattern} is defined as the maximum length of all possible patterns. Thus, the Dataset Volume is represented as the maximum between the size of \textbf{Vocabulary} and the size of \textbf{Pattern}, shown in line 5. From line 7 to line 13, after the while loop, the length of each list values under each key will be incremented $\gamma$ times with $\gamma - 1$ randomly shuffled values in total. From line 17 to 27, new sentences will be generated using each pattern $\rho$ stored in \textbf{Pattern} all required named entities $\o$, and $\o$ are elected from the \textbf{Vocabulary} using the \texttt{Pointer}. Each \texttt{Pointer} will be maintained to move within boundary of its belonging vocabulary $\eta$. 

Other augmentation approaches like \textbf{Pattern}-wise and \textbf{Vocabulary}-wise are also implemented for further comparison. The \textbf{Pattern}-wise augmentation promises all the \textbf{Pattern} within testing are unseen to the training process, and the \textbf{Vocabulary}-wise augmentation guarantees all \textbf{Vocabulary} in testing are unseen to the training process.

==> evaluation.tex <==
\section{Evaluation}

For evaluation propose, except metrics like Precision, Recall, Accuracy and F-1 score, Sentence-level Accuracy is introduced. Only when the model predicts the whole sentence correctly, the performance will be counted and the Sentence-level Accuracy will increase. 

original dataset w/ different parameter setting

augmented dataset 2, 5, 10, 100
default vocab pattern mixed

\textit{-----------Current Finding-----------}

Fail to achieve good performance on initial dataset

1. Default mode can give best results

2. Vocab: GloVe >> Self-generated embedding

3. Pattern: Self-generated embedding > GloVe

4. Training time: GloVe >> Self-generated embedding

5. Epochs taken: GloVe >> Self-generated embedding except on vocab mode

6. Seems harder for GloVe to converge(no embedding for PoS tags, which might lead to the zig-zaging on last several epochs)

Vanilla Seq2Seq~\cite{sutskever2014sequence} serves as a baseline model here for keyword extraction. In our design, the input is English sentences from user input; the output is a list of keywords following a predefined order, where all keywords are separated by dummy symbols. The predefined sequence is: `[Key1][Key2][Number][LocKey][Time]'. Using the same two sentences in Section 4, target sequences for both of the sentences will be like the following:
Target Sentence 1: `[concentration][TVOC][0.6 mg/m3][buildings][every day]';
Target Sentence 2: `[toluene][][0.2 mg per m3][park][]'.

Further both training and testing performance indicate the impotence of Seq2Seq when encountered with small datasets. Overall, the testing performance from Seq2Seq is 12\% on average and the training process shows an extremely high chance for the model to overfit. To tackle this, an early-stopping trick is applied, however, it still has trouble learning the key patterns from such a small dataset.

Meanwhile, the pretrained Stanford NLP NER~\cite{manning2014stanford} tagger is utilized to recognize all the Named Entities in this task. However, although the Stanford NER model yields success on some general datasets, we still find it task-specific. The general model, which gives only 3 output classes, and most of them have high data granularity. In this task, there are 5 output classes, and only the `LocKey' can be provided by the Stanford NER. Also, most of the 5 output classes are defined in a lower granularity level. To better meet the city-wise requirements, locations in this task are defined like `buildings' or `parks' instead of more general ones like `Shanghai' or `Tokyo'. Thus, assuming Stanford NER tagger can give us 100\% accuracy on the `LocKey' class, the overall domain-wise accuracy will not exceed 20\%.

\begin{center}
 \begin{tabular}{||c | c||} 
 \hline
 Model & Performance \\ [0.2ex] 
 \hline\hline
 Vanilla Seq2Seq & \ 11.956\% \\ 
 \hline
 Pretrained Stanford NER & \ 20\%* \\
 \hline
 BiLSTM + CRF & \ 62.52\% \\
 \hline
 BiLSTM + CRF with GloVe & \ 65.37\% \\
 \hline
\end{tabular}
\end{center}

As shown in the table above, both Vanilla Seq2Seq and Pretrained Stanford NER fail to generate a decent performance on this task. The Vanilla Seq2Seq model we implemented suffers a lot from data scarcity and begins to show signs of over-fitting after 5-10 training epochs, while the testing performance has not started to steadily increase yet. 

In the following evaluation experiments, we mainly focus on the influences of the proposed data augmentation approach on model performance. Our termination criteria are whether the model obtains a perfect training accuracy or not. 

\subsection{Time Efficiency}
Although BiLSTM + CRF with GloVe grants the model small advantages over the one without GloVe in terms of testing accuracy, the introduction of GloVe causes a lower time efficiency with more training epochs. The increased time by percentage after introducing GloVe is shown in the table below:

\begin{center}
 \begin{tabular}{||c | c | c||} 
 \hline
 Dataset & Time per epoch & Total time \\ [0.2ex] 
 \hline\hline
 Original Dataset & \ +14.28\% & +41.35\% \\
 \hline
 Random Augmented 100 & +3.85\% & +36.64\% \\
 \hline
 Vocab Augmented 100 & +12.5\% & +287.93\% \\
 \hline
 Pattern Augmented 100 & +3.85\% & +88.81\% \\
 \hline
 Mix(0.25) Augmented 100 & +4.76\% & +34.69\% \\
 \hline
 Mix(0.5) Augmented 100 & +2.38\% & +114.07\% \\
 \hline
 Mix(0.75) Augmented 100 & +78.57\% & +8.93\% \\
 \hline
\end{tabular}
\end{center}

The time spent each epoch increases by 2.38\% to 78.57\% and the overall time spent on training until the termination criteria are hit increases by 8.93\% to 287.93\%. On average, without GloVe, the model takes 38.57 epochs to hit the criteria, however, when GloVe is introduced, the number goes up to 55.42 which is creased by 43.7\%.

\subsection{Testing Performance}
With the strong prior knowledge of vocabulary from its designed training process, GloVe brings about significant advantages on augmented datasets with vocabulary-wise control.

\begin{center}
 \begin{tabular}{||c | c | c||} 
 \hline
 Dataset & CityEmbedding & GloVe \\ [0.2ex] 
 \hline\hline
 Original Dataset & \ 62.52\% & 65.37\% \\
 \hline
 Random Augmented 100 & 99.93\% & 88.49\% \\
 \hline
 Vocab Augmented 100 & 81.01\% & 88.49\% \\
 \hline
 Pattern Augmented 100 & 80.65\% & 81.58\% \\
 \hline
 Mix(0.25) Augmented 100 & 69.99\% & 74.47\% \\
 \hline
 Mix(0.5) Augmented 100 & 75.46\% & 74.47\% \\
 \hline
 Mix(0.75) Augmented 100 & 71.46\% & 78.34\% \\
 \hline
\end{tabular}
\end{center}

Meanwhile, introducing GloVe also gives a lower overall cover rate, which is around 92\% on average, due to its fixed vocabulary. The downgrade in cover rate is brought by the PoS tags. Because each sentence along with its corresponding PoS tags will be fed into the model as input. However, in the fixed vocabulary provided by pretrained GloVe, not all PoS tags are concluded. To vectorize all textual inputs, we have to assign those unseen PoS tags into a generic `UKN' class with some randomly generated representation. By doing so, it might cast some shadow during the training, since the model is confused by so many consecutive `UKN' in input. Observations(shown in figure 1) during the training models with GloVe tell that the model with GloVe although has a relatively impressive performance on word-level accuracy, it still struggles to hit the termination criteria and leads to a longer training time. This struggling is caused by the difficulty of learning detailed patterns from nested representation for all PoS tags.

\includegraphics[scale=0.1]{Figure/TrainAcc.png}

A huge leap in model performance, no matter is with or without GloVe, is observed after augmenting the original dataset. BiLSTM+CRF with GloVe has some more advantages while dealing with more unknown vocabulary in the testing set. However, when faced with more unknown patterns in the testing phase, the advantages brought by the introduction of GloVe become less obvious. 

However, We still note that the importance of masking all input tokens with separate representation vectors in improving time efficiency and model convergence. 

\subsection{Improvements from Data Augmentation}
In practical use, both absolute vocabulary-wise and pattern-wise control are extremely rare for users to encounter. Thus, we emphasize the improvements on the randomly-controlled augmented dataset with 100 as the augmentation index.  The following shows the performance differences in testing for the dataset size.

% Table \ref{tab:randomaugment}

% \tabref{}

 
\begin{table}
\caption{aaa (bbb)}
\footnotesize
 \begin{tabular}{||c | c | c||} 
 \hline
 Dataset & Without GloVe & With GloVe \\ [0.2ex] 
 \hline\hline
 Random Augmented 2 & 82.96\% & 79.71\% \\
 \hline
 Random Augmented 5 & 92.92\% & 91.19\% \\
 \hline
 Random Augmented 10 & 98.66\% & 97.51\% \\
 \hline
 Random Augmented 20 & 99.46\% & 99.07\% \\
 \hline
 Random Augmented 50 & 99.85\% & 99.76\% \\
 \hline
 Random Augmented 100 & 99.93\% & 88.49\% \\
 \hline
\end{tabular}
\label{tab:randomaugment}
\end{table}

\includegraphics[scale=0.04]{Figure/Size.png}

From the figure above, it is clearly shown the strong relationship between the size of augmented datasets with the proposed controllable augmentation process and the testing performances of both models with or without GloVe embeddings. The testing performance from the model without GloVe continuously increases when the size of the dataset reaches 100 bigger than the initial one. Meanwhile, the testing performance from the model with GloVe drops at the end.


% \begin{table*}[]
%     \centering
%     \begin{tabular}{c|c}
%          &  \\
%          & 
%     \end{tabular}
%     \caption{Caption}
%     \label{tab:my_label}
% \end{table*}

==> onlinelearning.tex <==
\section{Online Learning}
\label{sec:online}
Inspired by the Online Learning theory~\cite{hoi2018online} and its applications on Deep Learning platforms~\cite{sahoo2017online}, we separate the gained experiences into two parts: the Temporary Cache and the Permanent Knowledge. The Temporary Cache is devised to temporarily store those inputs that the deployed model is less confident at and the labels revealed by system users. By doing so the system can react fast with higher confidence while encountered with the same input in the future. The Permanent Knowledge is achieved by updating weights via back-propagation on the extended dataset with both initial data and the new input-label pairs stored in the Temporary Cache.

\subsection{Validation}

Data-driven approaches follow the garbage-in-garbage-out rule. Malicious input will damage the model performance. Malicious inputs can be `AAA' as LocKey in this setting. To keep our models away from malicious inputs, an additional validation process is needed after the user gives out the key-value pair and before the model inference.

\subsection{Acceptation and Rejection}

Here we introduce character-level models to filter those suspicious inputs based on previous inputs, which is defined as a classification task. The input of the model is the indicated inputs provided by the user and the output is one of those five key domains. 

Convolutional Neural Network is found to perform great in text classification tasks~\cite{Kim2014ConvolutionalNN}. Here we leverage the advantages that CNN brings in efficiency and key feature capture. Furthermore, based on the small size of the dataset and the relatively short length of the key-value pairs, a character-level more is more suitable for this task, since we are needing a light-weighted and easy-to-train solution. 

In addition, other neural structures like feed-forward neural networks, recurrent neural networks are also tried out to select the optimal solution for this task.

\begin{table}[h]
    \centering
        \caption{Validation Accuracy}
 \begin{tabular}{||c | c||} 
 \hline
 Model & Accuracy \\ [0.2ex] 
 \hline\hline
 Char-level \textbf{CNN} & \ xxx\% \\ 
 \hline
 Char-level RNN & \ xxx\% \\
 \hline
 Char-level FFN & \ xxx\% \\
 \hline
\end{tabular}
    \label{tab:ValAcc}
\end{table}

However, one unhappy case is when the model's output is different from the user's indication. In this case, the conflict can be understood as: this input tokens should be classified to another domain instead of the one provided by the user. We denote this type of fault as fault I.

If the model's output aligns with the key domain given by the user, it does not mean that the model is certain about the output. We call this type of fault II. In the neural network structure, we apply softmax as the final layer to gain the highest probability among the given five domains. By doing so, the softmax layer at the end is forcing the network to pick an answer from five given domains, no matter whether it is certain about it or not. To resolve this, Here we use a dropout layer that is set to be active during both training and testing to quantify the model uncertainty~\cite{ma2021predictive}. One trained model will be tested 100 times with the same dataset to test the model uncertainty about each testing sample. All samples produced by fault I and fault II will be rejected otherwise accepted.

During the experiments, we find the definitions of Key1 and Key2 depend on the whole sentence and it is harsh for the character-level model to tell the differences between Key1 and Key2 using that small amount of revealed information only. Even several words can be found both in Key1 and Key2. Here are some examples:

\begin{itemize}
    \item xxx
    \item xxx
\end{itemize}

Thus, we integrate the Key1 and Key2 to a new class called Key (for validation only) to experiment with the validation model.

\subsection{Simulated attacks}

To check the model's ability to tell the malicious attacks from others, we generate new samples from:

\begin{itemize}
    \item Randomly generated permutations of letters
    \item Some location names from other cities
    \item All units with randomly generated float numbers
\end{itemize}

Among all those newly generated samples, the validation model can give an accuracy of xxx. Among those are correctly predicted, the average confidence level is xxx. xxx samples are rejected because of fault I with the confidence of xxx and xxx samples are rejected because of fault II with the confidence of xxx.

\begin{figure}
    \centering
    \includegraphics[scale=0.5]{Figure/simlulated.png}
    \caption{Performance on simulated attacks}
    \label{fig:simulated}
\end{figure}

\subsection{Evaluation}

\textcolor{blue}{merge with Evaluation?}

After filtering all suspicious inputs, the model will be fine-tuned with newly validated samples.

A trained model after validated samples, performance goes up by xxx. But there is still a gap between the fully seen vocab.

A trained model after invalidated sample, performance might go up but not that obviously or even goes down by xxx.

